Principal Component Density Estimation for Scenario Generation Using Normalizing Flows

Neural networks-based learning of the distribution of non-dispatchable renewable electricity generation from sources such as photovoltaics (PV) and wind as well as load demands has recently gained attention. Normalizing flow density models are particularly well suited for this task due to the training through direct log-likelihood maximization. However, research from the field of image generation has shown that standard normalizing flows can only learn smeared-out versions of manifold distributions. Previous works on normalizing flow-based scenario generation do not address this issue, and the smeared-out distributions result in the sampling of noisy time series. In this paper, we exploit the isometry of the principal component analysis (PCA), which sets up the normalizing flow in a lower-dimensional space while maintaining the direct and computationally efficient likelihood maximization. We train the resulting principal component flow (PCF) on data of PV and wind power generation as well as load demand in Germany in the years 2013 to 2015. The results of this investigation show that the PCF preserves critical features of the original distributions, such as the probability density and frequency behavior of the time series. The application of the PCF is, however, not limited to renewable power generation but rather extends to any data set, time series, or otherwise, which can be efficiently reduced using PCA.

==> sections/99_Nomenclature.tex <==
\section*{Nomencalture}

\subsection*{Acronyms}
\noindent\begin{tabularx}{\columnwidth}{lX}
        ANN  & Artificial neural network      \\
        CEV  & Cumulative explained variance \\
        CVF  & Change of variables formula      \\
        DGM  & Deep generative model      \\
        FSNF & Full space normalizing flow    \\
        GAN  & Generative adversarial network   \\
        KDE  & Kernel density estimation      \\
        NICE & Nonlinear independent component estimation      \\
        PV   & Photovoltaic      \\
        PSD  & Power spectral density      \\
        PCA  & Principal component analysis      \\
        PCF  & Principal component flow      \\
        PDF  & Probability density function      \\
        RealNVP  & Real non-volume preserving transformation      \\
        VAE  & Variational autoencoder      \\
\end{tabularx}

\subsection*{Greek letters}
\noindent\begin{tabularx}{\columnwidth}{lX}
        $\theta$            & Trainable parameters of conditioner networks $s_\theta$ and $t_\theta$       \\
        $\mathbf{\mu}_X$    & Mean value of distribution $X$             \\
        $\psi$              & Injective transformation      \\
\end{tabularx}

\subsection*{Latin letters}
\noindent\begin{tabularx}{\columnwidth}{lX}
        $d$                 & Dimension                     \\
        $D$                 & Dimensionality of target distribution          \\
        $f$                 & Transformation                \\
        $f_{CL}$            & Coupling layer transformation \\
        $\mathbf{I}$        & Identity matrix               \\
        $\mathbf{J}$        & Jacobian                      \\
        $K$                 & Number of transformations in composition \\ 
        $M$                 & Dimensionality $<D$                \\
        $p_X/p_Y$           & Probability density of $X$ and $Y$\\
        $s_\theta$          & Conditioner network           \\
        $t_\theta$          & Conditioner network           \\
        $\mathbf{V}$        & Matrix of right singular vectors \\        
        $\mathbf{V}_P$      & Truncated matrix of right singular vectors \\
        $\mathbf{x}$        & Target distribution sample    \\
        $\mathbf{\tilde{x}}$& Compressed target distribution sample   \\
        $X$                 & Target distribution           \\
        $\mathbf{z}$        & Base distribution sample      \\
        $Z$                 & Base distribution             \\
\end{tabularx}
